(2+1)-Einstein spacetimes of finite type

The aim of this survey is to give an overview on the geometry of Einstein maximal globally hyperbolic 2+1 spacetimes of arbitrary curvature, conatining a complete Cauchy surface of finite type. In particular a specialization to the finite type case of the canonicla Wick rotation-rescaling theory, previously developed by the authors, is provided. This includes, for arbitrary curvatures, parameterizations in terms of suitable measured geodesic laminations on open hyperbolic surfaces of finite type. The same geometric objects also parameterize complex projective structures on the surfaces. The coincidence of such parameter space is explained by means of geometric correlations between spacetimes of different curvatures and projective surfaces realized via canonical WR-rescaling along the cosmological times. We also specialize on AdS case mostly referring to recent results achieved by other authors. In particular we describe maximal causal extensions of AdS globally hyperbolic spacetimes and an AdS approach to the theory of earthquakes for hyperbolic surfaces of finite type. A general earthquake theorem is proved for the so called enhanced Teichmuller space. The case of spacetimes with conical timelike singularities is also treated.

==> HANDBH.tex <==
\section{AdS causal extensions, earthquakes and black holes}\label{BH}
Let $M$ be an AdS maximal globally hyperbolic spacetime containing a Cauchy
surface $S$. The holonomy of $M$, say $h=(h_L,h_R):\pi_1(S)\rightarrow
PSL(2,\mr)\times PSL(2,\mr)$, is formed by a pair of discrete and faithful
representations of $\pi_1(S)$ into $PSL(2,\mr)$ such that $\mh^2/h_L\cong
\mh^2/h_R\cong S$. Moreover, the developing map is an isometric embdedding,
so $\tilde M$ can be identified with some open (and convex) set of $\mx_{-1}$.

If $S$ is closed,  $\tilde M$, as subset of $\mx_{-1}$, is
determined by $h$. Indeed a point $x\in\mx_{-1}$ lies in $\mx_{-1}$ iff its
translates by $\pi_1(S)$ are not related to $x$ by any timelike geodesic.
As a consequence, we have that $M$ is determined by its holonomy.

When $S$ is not compact the picture is a bit different. In fact, we
can consider the domain, say $\tilde\Omega(h)$, of points whose
translates by $\pi_1(S)$ are not causally related to $x$.  Barbot
proved that the action of $\pi_1(S)$ on $\tilde\Omega(h)$ is free and
properly discontinuous and the quotient, say $\Omega(h)$, is a causal
Lorentzian manifold homeomorphic to $S\times\mr$. Since $M$ is causal,
$\tilde M\subset\tilde\Omega(h)$, but the inclusion is in general
strict. The reason is that the adherence,
$\partial_\infty\tilde\Omega(h)$, of $\tilde\Omega(h)$ on the boundary
of $\mx_{-1}$ has non-empty interior part. Such an adherence can be
explicitly described by means of the holonomy of the peripheral loops.
For every $\gamma\in\pi_1(S)$ parallel to a puncture let $I_L(\gamma)$
(resp.  $I_R(\gamma)$) be the interval of $S^1$ whose end-points are
the fixed points of $h_L(\gamma)$ (resp. $h_R(\gamma)$) and that does
not meet the limit set of $h_L(\gamma)$ (resp. $h_R(\gamma)$). If
$h_L(\gamma)$ is parabolic, then let $I_L(\gamma)$ be the fixed point
of $h_L(\gamma)$. Then the rectangle $R(\gamma)=I_L(\gamma)\times
I_R(\gamma)$ is contained in the adherence of $\tilde\Omega(h)$, and
in fact $\partial_\infty\tilde\Omega(h)$ is the closure
$\bigcup_\gamma R(\gamma)$. The closure of the complementary of
rectangles $R(\gamma)$ in $\partial_\infty\tilde\Omega(h)$ can be
ragarded as a limit set, in the sense that it is contained in the
closure of the orbit of any point $x\in\overline{\mx_{-1}}$.

If some rectangle $R(\gamma)$ is not degenerate (that is, both
$h_L(\gamma),h_R(\gamma)$ are hyperbolic), then the interior of
$\partial_\infty\tilde\Omega(h)$ is not empty. As a consequence,
$\Omega(h)$ is not globally hyperbolic: indeed it is possible to find
points $p,q$ close to $R(\gamma)$ such that $\fut(p)\cap\pass(q)$ is
not pre-compact in $\mx_{-1}$ and this contradicts the global
hyperbolicity.

On the other hand, for any point $p\in\tilde\Omega(h)$, it is possible
to find a complete spacelike surface $\Sigma_p$ containing $p$ and
invariant under $\pi_1(M)$. The domain of dependence of $\Sigma_p$,
say $D(\Sigma_p)$, is globally iperbolic and invariant under $h$. It
follows that $D(\Sigma_p)\subset\Omega(h)$. So we can briefly say that
$\Omega(h)$ is the union of GH spacetimes whose holonomy is $h$.

In Physics literature the space $\Omega(h)$  is known as a multi black hole. 
More precisely, the black hole
$B(h)$ is the set of points causally disconnected from the asymptotic
boundary, that is the universal covering $\hat B(h)$ is 
the set of points such that lightlike rays emanating from
them do not reach $\partial_\infty\Omega(h)$. It turns out that $B(h)$ is the
intersection of the domain of dependence of complete spacelike surfaces
contained in $\Omega(h)$. Thus, $B(h)$ can be
regarded as the intersection of all GH spacetimes whose holonomy is $h$.

The black hole disconnects $\Omega(h)$ into some regions called
\emph{asymtotic regions}. In the universal covering, the adherence of
each asymtotic region in $\partial_\infty\Omega(h)$ is a
non-degenerate rectangle, and for each non-degenerate rectangle there
is exactly one asymtotic region that bounds it.  So to the quotient
there are $k$ region where $k$ is the number of punctures that appear
geodesic boundaries in both $\mh^2/h_L$ and $\mh^2/h_R$.  The
asymtotic region corresponding to $R(\gamma)$ will be denoted by
$A(\gamma)$

In the universal covering, every asymptotic region, $\tilde
A(\gamma)$, is separated from $\tilde B(h)$ by a surface, called an
\emph{horizon} of $\tilde B(h)$, that is the union of two lightlike
planes intersecting along a spacelike geodesic. Such a geodesic is
invariant for $(h_L(\gamma),h_R(\gamma))$. So the quotient $\partial
A(\gamma)$ is the union of two lightlike annuli along a spacelike
geodesic. The length of this spacelike geodesic is called the
\emph{size} of the horizon, whereas the \emph{momentum} is the twist
factor for the parallel transfort along it.  If $l_L,l_R$ are the
translation lengths of $h_L(\gamma)$ and $h_R(\gamma)$, the size of
the black hole is simply $(l_L+l_R)/2$ whereas the momentum is
$(l_L-l_R)/2$.

\subsection{BTZ-black hole}\label{BTZ}

\subsection{Bent surfaces in $\Omega(h)$}
In~\cite{M} it has been shown that a MGH AdS spacetimes contains
exactly two bent convex hyperbolic surfaces that are the boundary
components of its convex core (actually they coincide in the static
case).

On the other hand, since $\Omega(h)$ contains many MGH spacetimes, it
contains many bent convex hyperbolic surfaces. Let us remark the set
of MGH spacetimes whose holonomy is $h$ and that contain a complete
Cauchy surface is in $1$-to-$1$ correspondence with the set of
$h$-invariant no-where timelike meridians in $\partial\mx_{-1}$. This
correspondence associates to a spacetime $M$ the adherence on the
boundary $\partial_\infty\tilde M$ of the universal covering of $M$
(regarded as a $h$-invariant subset of $\mx_{-1}$).

On the other hand each meridian contained in $\partial_\infty\Omega$
is determined by drawing in each rectangle $R(\gamma)$ an arc
$l_\gamma$ joining the vertices that are the end-points of the core of
the horizon corresponding to $\gamma$ (in the degenerate case the
segment $l_\gamma$ coincide with $R(\gamma)$). The closure $L$ of the
union of $l_\gamma$ is a meridian, and if the segments are chosen in a
$\pi_1(M)$-invariant way (that is
$l_{\alpha\gamma\alpha^{-1}}=h(\alpha) l_\gamma$), then $L$ is
$\pi_1(M)$-invariant, so its Cauchy development is
$\pi_1(M)$-invariant.

A case of particular interest is when the segments $l_\gamma$ are chosen on
the boundary of $R(\gamma)$. Meridians obtained in this way are called
extremal.  Notice that for each asymtotic region there are only two ways to
chose such an arc: an upper extremal arc and a lower extremal arc. 
Thus, there are $2^k$ $\pi_1(M)$-invariant extremal arcs
where $k$ is the number of non-degenerate rectangles up to $\pi_1(M)$.

The bent convex surfaces of $\Omega(h)/h$ corresponding to extremal
$\pi_1(M)$-invariant meridians have a nice carachterization in geometric
terms. In fact, they are the only bent convex surfaces of $\Omega(h)/h$ that
intrinsically are structures in $\Tt_\Cc(S)$. 

\subsection{Earthquakes of surfaces with geodesic boundaries}\label{BH_quake}
Given a MGH spacetime $M$ containing a closed surface $S$, with
holonomy $h=(h_L, h_R)$, let $F_+,F_-$ be the bent hyperbolic surface
conatined in $M$ resepctively past and future convex. Denote by
$\lambda_\pm$ the respctive bending laminations. In~\cite{M} it has
been proved that $\mh^2/h_R$ is obtained by a left earthquake on $F_+$
along $\lambda_+$ (and by a right earthquake on $F_-$ along
$\lambda_-$). Anagolously the right earthquake on $F_+$ along
$\lambda_+$ produces $\mh^2/h_L$ (and by a left earthquake on $F_-$
along $\lambda_-$).

This relation between AdS geometry and earthquake theory gives a new
evidence of the existence (and uniqueness) of a left earthquake
joining any pair of points in the Teichmuller space of $S$. Indeed,
given two hyperbolic structures with holonomies $h_L,h_R$, one can
consider the MGH spacetime $M$ whose holonomy is the pair
$(h_L,h_R)$. If $\lambda_+$ is the bending lamination of the
past-convex bent surface in $M$, then the above picture show that the
left earthquake along $2\lambda_+$ connects $\mh^2/h_L$ to
$\mh^2/h_R$.

Conversely if the left earthquake along $\lambda$ connects $\mh^2/h_L$
to $\mh^2/h_R$, then the surface, say $F$, obtained by a left
earthquake along $\lambda/2$ on $\mh^2/h_L$, can be obtained as a
past-convex bent surface in $M$ with bending lamination
$\lambda/2$. Thus $F=F_+$ and $\lambda/2=\lambda_+$.

The same arguments, when $S$ is assumed only to be of finite type,
lead to prove Theorem~\ref{quake-teo}

Indeed let $h_L,h_R$ two discrete and faithful representations of
$\pi_1(S)$ into $PSL(2,\mr)$ such that $\mh^2/h_L\cong\mh^2/h_R\cong
S$. Denote by $\Omega(h)$ the corresponding MBH. A past-convex
hyperbolic surface $F_+$ in $\Omega(h)$ bent along a measured geodesic
lamination $\lambda_+$, is transformed by a left (resp. right)
earthquake along $\lambda_+$ into a hyperbolic surface $F_L$
(resp. $F_R$) whose holonomy is $h_L$ (resp. $h_R$).  Anyway in
general $F_L$ is only a surface with geodesic boundary but it does not
coincide with $\mh^2/h_L$ nor with its convex core.  On the other hand
$F_L$ coincides with the convex core of $\mh^2/h_L$ iff

1. $F_+$ has finite area 

2. The gedesic boundary of $F_+$ is compact. 

The reason why these conditions are sufficient is that if $F_+$
satisfies them, then so does any surface obtained by a left (or right)
earthquake on $F_+$. On the other hand the convex core of $\mh^2/h_L$
is the only hyperbolic surface contained in $\mh^2/h_L$ satisfying
them.

From the previous subsection we know that $F_+$ satisfies to
conditions 1. and 2. iff it corresponds to an extremal meridian in
$\partial\mx_{-1}$.


Let us analyze more deeply the lack of uniqueness.  Let $\lambda$ be a
measured geodesic lamination spiralling around a boundary component
$c$ of $F_L$, and denote by $F_t$ the hyperbolic surface obtained by a
left earthquake along $t\lambda$. The length of $c$ with respect to
$F_t$ depends linearly on $t$ with slope whose absolute value is
$I_\lambda(c)$ (notice that for a non-peripheral loop, $l_t(c)$ is
either constant, corresponding to the case $c\cap\lambda=\varnothing$,
or strictly convex).


There are two possibilities. Either $\lambda$ spirals in a positive
way around $c$, or in a negative way.  In the former case
$I_\lambda(c)$ is stricly positive, so the length of $c$ grows more
and more along the earthquake past $t\mapsto F_t$.

In the latter case $I_\lambda(c)$ is strictly negative. So the length
of $c$ decreases until $c$ collapses to a cusp (that happens at time
$t_0=l_0(c)/|I_\lambda(c)|$).  After that critic time the length
increases linearly with slope $-I_\lambda(c)$. If $\lambda_t$ denotes
the image of $\lambda$ in $F_t$ via the left earthquake, it turns out
that $\lambda_t$ spirals in the negative way around $c$ for $t<t_0$
whereas spirals in the positive way for $t>t_0$ (notice that for
$t=t_0$ it does enter the cusp without spiralling).

This picture suggests the idea that at time $t_0$ there is a kind of
bouncing in the Teichmuller space $\Tt_C(S)$. Moreover it lead to lift
the earthquake flow on $\Tt_C^\#(S)$ as we did in
Section~\ref{bend-quake}. Corollary~\ref{nec-comp} and
Theorem~\ref{quake-teo} easily descend from previous remarks.

\subsection{Convex core of a Black Hole}\label{BH_convexcore}
We have seen there exists a minimal closed subset
$\Lambda\subset\partial\mx_{\infty}$ invariant under
$h=(h_L,h_R)$. Its convex core is contained in $\tilde\Omega(h)$ and
produces to the quotient the minimal convex retract of $\Omega(h)$
that is called its convex core. The convex core $\Kk(h)$ is contained
in $B(h)$. It is interesting to study the boundary of $\Kk(h)$. It
contains the spacelike geodesics of the horizons of $B(h)$. Such
geodesics disconnects $\partial\Kk(h)$ into two surfaces homeomorphic
to $S$. One is convex in the past and the other one is convex in the
future. Denote by $\partial_+\Kk(h)$ the former one and by
$\partial_-\Kk(h)$ the latter one. Now $\partial_+\Kk(h)$ is
intrinsically a hyperbolic surface bent along a measured geodesic
lamination. Its area is finite and its boundary components are the
closed geodesics of the horizons. So
$\partial_+\Kk(h)\in\Tt_\Cc(S)$. in particular its number of boundary
components is equal to $k$, where $k$ is the number of punctures $c$
of $S$ such that $h_L(\gamma)$ and $h_R(\gamma)$ are both hyperbolic
for some representative $\gamma$ of $c$.

The extremal curve in $\partial\mx_\infty$ corresponding to $\partial_+\Kk(h)$
(resp- $\partial_-\Kk(h)$) is obtained by taking the lower (resp. upper)
extremal arc in each rectangle.

For each boundary component $c_i$ of $\partial_+(\Kk)$, we have that $l(c_i)$
is the size of the corresponding horizon, whereas $I_{\lambda_+}(c_i)$ is the
corresponding momentum. It follows that $\lambda_+\in\Vv^*(\partial_+\Kk(h))$.
In fact this property characterizes $\partial_+\Kk(h)$ in the sense that
 it is the unique bent surface in $\Omega(h)$ such that its bending lamination
 lies in $\Vv^*$.

As a consequence we have that given two points in $\Tt_C(S)$, say $F_L,F_R$
with holonomies $h_L,h_R$, there is a unique left earthquake connecting them
without bouncing. Its shearing locus corresponds to the (double of) the
bending locus of the upper boundary of the convex core of $\Omega(h)$.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "HAND"
%%% End: 

